Automated Deep Learning Optimization via DSL-Based Source Code Transformation

As deep learning models become increasingly bigger and more complex, it is critical to improve model training and inference efficiency. Though a variety of highly optimized libraries and packages (known as DL kernels) have been developed, it is tedious and time-consuming to figure out which kernel to use, where to use, and how to use them correctly. To address this challenge, we propose an Automated Deep learning OPTimization approach called Adopter. We design a Domain-Specific Language (DSL) to represent DL model architectures and leverage this DSL to specify model transformation rules required to integrate a DL kernel into a model. Given the source code of a DL model and the transformation rules for a set of kernels, Adopter first performs inter-procedural analysis to identify and express the model architecture in our DSL. Then, Adopter performs scope analysis and sub-sequence matching to identify locations in the model architecture where the transformation rules can be applied. Finally, Adopter proposes a synthesis-based code transformation method to apply the transformation rule. We curated a benchmark with 199 models from Hugging Face and a diverse set of DL kernels. We found that, compared to a state-of-the-art automated code transformation technique, Adopter helps improve the precision and recall by 3% and 56%, respectively. An in-depth analysis of 9 models revealed that on average, Adopter improved the training speed by 22.7% while decreasing the GPU memory usage by 10.5%.

==> templates/0-Abstract.tex <==
\begin{abstract}
Automated Program Repair (APR) holds the promise of alleviating the burden of debugging and fixing software bugs. Despite the great stride in advancing APR algorithms, the usability of APR techniques remains a largely unexplored area. One major usability challenge lies in understanding and trusting auto-generated patches. This challenge is exacerbated in the presence of plausible patches since developers need to manually inspect each of them and identify the correct one, which is tedious and time-consuming. To address this challenge, we propose an interactive approach called {\iFix} that allows developers to quickly explore a large number of patch candidates and examine their behavior difference without manual debugging. To enable such interactions, we develop (1) a new multi-criteria sampling and re-ranking algorithm that selects a small set of diverse and representative patches and establishes a hierarchy among remaining patches for ease of navigation and (2) an automated behavior analysis approach that identifies variables related to the given bug and log their runtime values for comparison. 
The quantitative experiment shows that our multi-criteria method can improve the ranking of correct patches by at least 34\% compared with APR tools and other ranking methods.
We have implemented {\iFix} as a Visual Studio Code extension and conducted a within-subjects user study with 15 participants. Compared with manual debugging and a state-of-the-art patch filtering technique, {\iFix} improves the success rate by \UserSuccessRateBoostAgainstManual and \UserSuccessRateBoostAgainstBaseline while reducing the task completion time by \UserDebugTimeReducedAgainstManual and \UserDebugTimeReducedAgainstBaseline, respectively. 
\end{abstract}


==> templates/1-Introduction.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{./Figures/overview.pdf}
    % \precaptionspace
    %\vspace{-2ex}
    \caption{A System Overview of \iFix}
    % \vspace{-2ex}
    \label{fig:ifix-framework}
\end{figure*}

Program repair is a crucial yet challenging and time-consuming task in software development. A recent survey with 950 developers finds that more than a third of developers spent up to a quarter of their time fixing software bugs, while 44\% of developers identified bug fixing as their biggest pain point in software development~\cite{2021survey}. Automated Program Repair (APR) is a promising research area that aims to replace or supplement the manual bug-fixing process. Over the past decade, various APR techniques have been proposed, spanning across template-based, search-based, heuristics-based, and learning-based methods~\cite{le2011genprog, saha_elixir_2017,xuan_nopol_2017,hua_sketchfix_2018,wen_context-aware_2018, marginean_sapfix_2019, bader2019getafix, mechtaev2016angelix}. 
%Kim and Whitehead [14] report that the median time for fixing a single bug is about 200 days~\cite{kim2006long}.
So far, state-of-the-art APR techniques have achieved a bug-fixing rate up to \SotaAPRFixRateDefects~\cite{xia_less_2022} on Defects4J~\cite{just2014defects4j} and \SotaAPRFixRateQuixBug~\cite{jiang_cure_2021} on QuixBugs~\cite{lin_quixbugs_2017}. 

Despite this great stride, usability remains a major challenge for adopting APR techniques in practice~\cite{long_analysis_2016, izquierdo-cortazar_are_nodate, winter_how_2022, zhang_program_2022, winter_lets_2023, noller_trust_2022, zhong_empirical_2015}.  
Previous studies have shown developers are skeptical of the quality and correctness of automatically generated patches, leading to significant effort to review and verify those patches~\cite{long_analysis_2016, zhong_empirical_2015, noller_trust_2022}. This issue is exacerbated by the presence of plausible but unnecessarily correct patches~\cite{long_analysis_2016}, since developers need to carefully examine each patch candidate to identify the correct one. To help developers build trust on automatically generated patches, an efficient patch assessment is crucial and often desired by developers~\cite{noller_trust_2022, long_analysis_2016}. Specifically, Noller et al.~\cite{noller_trust_2022} find that developers want to see evidence for patch correctness, such as runtime behavioral information, to efficiently understand the root cause of a bug and select patch candidates. % and \Comment{the exact buggy locations~\cite{tao_automatically_2014}, additional context information related to the buggy code base (i.e. extra test cases)~\cite{noller_trust_2022}, as well as}
% Furthermore, it is critical to provide aid to help understand the root cause of bugs and distinguish between patches~\cite{cambronero_characterizing_2019}. %Studies on human developers indicated that the extent to which APR-generated patches can help improve the efficiency and precision of fixing real software bugs depends on various factors~\cite{tao_automatically_2014, winter_lets_2023, winter_how_2022} including the difficulty of bugs, the quality of patches, the knowledge level of programmers, etc. Meanwhile, this effect is not always positive~\cite{cambronero_characterizing_2019, winter_lets_2023, zhang_program_2022}. These findings calls for more focus on providing solutions for developers to make use of the patches generated by APR techniques.

%While APR techniques have been increasingly adopted in the industry to reduce the cost of debugging and fixing bugs~\cite{harman_finding_2018, marginean_sapfix_2019}, 
% there are a few studies on developing and evaluating interactive tools to help developers fixing bugs with the aid of APR-generated patches. Liang et al. suggested that classifying patches based on their different location in the code base, their affections on the control flow and their affections on return value of functions can help developers filter out incorrect patches in a shorter time.~\cite{liang_interactive_2021} Zhang et al. claimed that it is more likely to build trust between developer and APR-generated patches if additional test cases are provided. ~\cite{zhang_interactive_2022}.


% There are a few interactive approaches based on generating test cases (e.g. HUGO~\cite{zhang_interactive_2022}, Learn2Fix~\cite{bohme_2020_human}) to help developers debug their programs with the aid of APR techniques. While these tools introduce extra test cases, 
Recently, several interactive approaches have been proposed to involve developers in the automated program repair process~\cite{liang_interactive_2021, bohme_2020_human, cashin2019understanding, gao2020interactive}. While Böhme et al.~\cite{bohme_2020_human} and Gao and Roychoudhury~\cite{gao2020interactive} aim to elicit human feedback to guide the patch generation process, Cashin et al.~\cite{cashin2019understanding} and Liang et al.~\cite{liang_interactive_2021} provide interactive support for patch filtering. Specifically, Cashin et al.~\cite{cashin2019understanding} propose to infer invariants from patches and then cluster semantically similar patches based on their invariants. Though clustering can reduce the number of patches to examine, it does not eliminate the need for debugging patches and comparing the behavioral difference of patches from different clusters. Liang et al.~\cite{liang_interactive_2021} help developers examine the behavioral difference between  patches by rendering their execution traces side by side, along with the runtime values at the entry and exit locations of patched methods. However, their approach does not scale to more than two patches. Furthermore, only rendering runtime values at the entry and exit of patched methods is not sufficient to help developers fully understand the behavior and runtime impact of a patch, since developers still need to manually figure out how the runtime values flow from the buggy statement to the test assertion in order to understand how the bug is fixed.  

In this work, we propose an interactive approach called \emph{iFix} to help developers examine the behavior difference among multiple patch candidates and select the correct one without manual debugging. Figure~\ref{fig:ifix-framework} gives an overview of {\iFix}. Previous studies have shown that users prefer to inspect a small number of high-quality patches, rather than a large number of patches that are potentially correct~\cite{noller_trust_2022, zhong_empirical_2015}. Thus, \iFix employs a \emph{multi-criteria sampling \& re-ranking} method, which selects a small set of diverse and representative patches and establishes a cluster hierarchy among the remaining patches. 
% This approach can be applied repeatedly on any cluster within the hierarchy as long as it has enough patches to be further classified.
Building upon this method, \iFix provides interactive support to allow developers to actively inspect a few patches and dive into promising ones while excluding nonsensical ones to explore a large patch space. 

Furthermore, to help developers compare the runtime behavior across multiple patches, we develop a new behavioral analysis method that automatically identifies variables related to a given bug, instruments the code to capture their runtime values, and aligns them across patches in a behavior comparison table. \iFix also captures the runtime values across the call stack trace of the buggy code and renders how  faulty values propagate from the buggy code to the test assertion to help developers understand the root cause of the bug and how it is fixed by different patches. We have implemented {\iFix} as an extension in Visual Studio (VS) Code. Figure~\ref{fig:ui-overview} shows the user interface of {\iFix}. %It enables \iFix to provide a {\em Behavior Comparison Table} that displays the runtime values of multiple versions of code bases side by side. 
%\lin{to me, this is one of the most important contributions of iFix. Does InPaFar and other tools have Runtime Behavior Comparison? If not, we should emphasize this contribution. Although someone can  use existing patch clustering techniques to group patches, they still need to debug and validate each patch one by one. iFix enables developers to see the debugging info from multiple patches and executions side by side, which is novel and should significantly improve the effectiveness and efficiency of patch selection and validation }\ruixin{Added to contributions.}
% To provide additional information to help users compare the runtime behavior of the source code under different patches, \iFix provides a \emph{Runtime Behavior Comparison table}. We managed to log runtime values (i.e. variables, method calls, infix expressions) by adopting code instrument based on results of code analysis. We introduced some handy utilities on \iFix to make it more user-friendly. 


To evaluate \iFix, we conducted a quantitative study to measure the performance of our multi-criteria sampling and re-ranking algorithm and a within-subjects user study to evaluate the usefulness and usability of \iFix. Our quantitative experiment shows that our multi-criteria can improve the overall ranking of correct patches by at least 34\% compared with the original ranking of APR tools, static-feature-based ranking techniques, and the learning-based ranking method. Our user study with 15 participants demonstrates that {\iFix} can significantly improve the patch selection correction and efficiency compared to two baselines---manual debugging and selecting patches and InPaFer, a state-of-the-art interactive patch filtering  technique~\cite{liang_interactive_2021}. Specifically, compared with the two baselines, {\iFix} improves the success rate of patch selection by  \UserSuccessRateBoostAgainstManual and \UserSuccessRateBoostAgainstBaseline while reducing task completion time by 37\% and 38\%, respectively. %(2) Due to the variety of the programming knowledge of our participants, \iFix has the best affect when the participant tend to use debugger when fixing bugs without any tool but a list of APR-generated patches.

Overall, our work makes the following contributions:

\begin{itemize}[leftmargin=0.6cm]

  \item   We proposed a new multi-criteria sampling and re-ranking algorithm to reduce the effort of inspecting many patch candidates.
  \item we proposed a new runtime behavior analysis method that automatically analyzes and instruments both buggy and patched code to capture their runtime behavioral differences along the call stack trace.
  \item Building upon the two new methods, we developed an interactive approach called \iFix and implemented it as a VS Code extension to help developers navigate, examine, and select automatically generated patches. 
  \item We conducted both qualitative experiments and user studies to evaluate the effectiveness of our sampling and re-ranking algorithm and the overall usefulness of \iFix compared to multiple baselines. The insights gained from this evaluation have the potential to inform future research in this area.
\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:MotivatingExample} motivates the problem with a real-world example. Section \ref{sec:Methodology} describes two key methods that empower {\iFix}.  Section \ref{sec:UserInterface} describes the user interface design of \iFix. Section \ref{sec:QuantitativeExperiment} describes a quantitative evaluation on our multi-criteria sampling \& re-ranking method. Section \ref{sec:UserStudy} describes a user study that evaluates the usefulness and usability of \iFix. Section \ref{sec:Discussion} discusses the potential avenues for future research and the threats to the validity. Section \ref{sec:RelatedWork} discusses related work, and Section \ref{sec:Conclusion} concludes the paper. Our code and data have been made available in an anonymous GitHub repository for review.\footnote{\href{https://anonymous.4open.science/r/iFix}{https://anonymous.4open.science/r/iFix}} 

==> templates/2-MotivatingExample.tex <==
%New colors defined below
\definecolor{codegreen}{rgb}{0.13,0.41,0.24}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.52,0.03,0.40}
\definecolor{backcolour}{rgb}{1.0,1.0,1.0}


%Code listing style named "mystyle"
\lstdefinestyle{code}{
  backgroundcolor=\color{backcolour},
  commentstyle=\color{codegreen},
  keywordstyle=\color{codepurple},
  numberstyle=\tiny\color{codegray},
  stringstyle=\color{magenta},
  basicstyle=\ttfamily\footnotesize,
  breakatwhitespace=false,         
  breaklines=true,                 
  captionpos=b,                    
  keepspaces=true,                 
  numbers=left,                    
  numbersep=5pt,                  
  showspaces=false,                
  showstringspaces=false,
  showtabs=false,                  
  tabsize=2,
  escapeinside=||
}
% \lstset{style=code}

\lstset{numbers=left, numberblanklines=false, escapeinside=||, style=code}
\let\origthelstnumber\thelstnumber
\makeatletter
\newcommand*\Suppressnumber{%
  \lst@AddToHook{OnNewLine}{%
    \let\thelstnumber\relax%
     \advance\c@lstnumber-\@ne\relax%
    }%
}

\newcommand*\Reactivatenumber[1]{%
  \setcounter{lstnumber}{\numexpr#1-1\relax}
  \lst@AddToHook{OnNewLine}{%
   \let\thelstnumber\origthelstnumber%
   \refstepcounter{lstnumber}
  }%
}

\makeatother


\Comment{\begin{figure}[hbtp]
\vspace{4pt}
\raggedright{\CodeIn{MannWhitneyUTest.java}}
\vspace{2pt}
\hrule
\begin{lstlisting}[language=Java, firstnumber=168]
private double calculateAsymptoticPValue(final double Umin, final int n1, final int n2)|\Reactivatenumber{170}|
    throws ConvergenceException, MaxCountExceededException {         |\Suppressnumber||\Reactivatenumber{172}|
    final int n1n2prod = n1 * n2;           /* buggy */  |\Suppressnumber||\Reactivatenumber{175}|
    final double EU = n1n2prod / 2.0; |\Suppressnumber||\Reactivatenumber{176}|
    final double VarU = n1n2prod * (n1+n2+1) / 12.0; |\Suppressnumber||\Reactivatenumber{178}|
    final double z = (Umin-EU) / FastMath.sqrt(VarU);|\Suppressnumber||\Reactivatenumber{180}|
    final NormalDistribution standardNormal = new NormalDistribution(0, 1);|\Suppressnumber||\Reactivatenumber{182}|
    return 2 * standardNormal.cumulativeProbability(z);|\Suppressnumber||\Reactivatenumber{183}|
}\end{lstlisting}
\hrule
\begin{lstlisting}[language=Java, firstnumber=217]
public double mannWhitneyUTest(final double[] x, final double[] y)|\Suppressnumber||\Reactivatenumber{218}|
    throws NullArgumentException, NoDataException,|\Suppressnumber||\Reactivatenumber{219}|
    ConvergenceException, MaxCountExceededException {|\Suppressnumber||\Reactivatenumber{221}|
    ensureDataConformance(x, y);|\Suppressnumber||\Reactivatenumber{223}|
    final double Umax = mannWhitneyU(x, y);|\Suppressnumber||\Reactivatenumber{228}|
    final double Umin = x.length * y.length - Umax;|\Suppressnumber||\Reactivatenumber{230}|
    return calculateAsymptoticPValue(Umin, x.length, y.length);|\Suppressnumber||\Reactivatenumber{231}|
}\end{lstlisting}
\raggedright{\CodeIn{MannWhitneyUTestTest.java}}
\vspace{2pt}
\hrule
\begin{lstlisting}[language=Java, firstnumber=105]
public void testBigDataSet() throws Exception {
    double[] d1 = new double[1500];
    double[] d2 = new double[1500];|\Suppressnumber|
    ...|\Reactivatenumber{112}|
    double result = testStatistic.mannWhitneyUTest(d1, d2);
    Assert.assertTrue(result > 0.1);
}\end{lstlisting}
\hrule
\caption{Code Snippets of Bug Math 30 in Defects4J}
\label{fig:codebase-1}
\end{figure}}




This section motivates \iFix with a bug from the Apache Commons Math project (Math 30 from Defects4J~\cite{just2014defects4j}). Suppose Alice is a developer who makes contributions to the Apache open-source community. She is assigned to fix this bug. Figure \ref{fig:codebase-1} shows the buggy method (\CodeIn{MannWhitneyUTest.calculateAsymptoticPValue}) and the test case (\CodeIn{MannWhitneyUTestTest.testBigDatasSet}). The \CodeIn{calculateAsymptoticPValue} method computes the asymptotic p-value via normal approximation. The unit test, \CodeIn{testBigDataSet}, aims to test \CodeIn{MannWhitneyUTest} with an input of two data samples consisting of 1500 integers. It fails since the p-value calculated by this method is a number greater than an expected value, $0.1$. The buggy statement is located at Line\#173 in \CodeIn{calculateAsymptoticPValue}, which  calculates the production of two integers.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/codesnippet.png}
    % \precaptionspace
    \caption{Code Snippets of Bug Math 30 in Defects4J}
    \label{fig:codebase-1}
\end{figure}

%As the codebase of this large project involves contributions from hundreds of developers, Alice was not familiar with the code corresponding to the bug. 
The code in \CodeIn{MannWhitneyUTest.java} was written by another developer who is no longer active in the open-source community. Since Alice is unfamiliar with the code as well as the underlying statistics in Mann Whitney U Test, she decides to try an APR tool first and check whether it can generate any inspiring patches to help her fix this bug. Indeed, the APR tool successfully generates 33 plausible patches after running for a while, as shown in Table~\ref{table: example-patches}. All these 33 patches fix the test failure in \CodeIn{MannWhitneyUTestTest.testBigDatasSet} without introducing another failure. Alice is impressed, but she also realizes that some patches seem to fix the bug simply by coincidence after a glance.  
%However, many of these patches just made the test cases pass by coincidence~\cite{smith_is_2015, le_overfitting_2018} and thus are not correct.

\begin{table}[h]
 
\small
  {%
    \caption{The auto-generated plausible patches, with the correct one marked with $\star$}
    \label{table: example-patches}
    %\vspace{-2ex}
  \begin{tabular}{cc}
    \toprule
    Index & APR-Generated Patches\\
    \midrule
    \ \ \ \ 1 & \CodeIn{double n1n2prod = n1*( n2+ n2) /2.0;}\\
    \ \ \ \ 2 & \CodeIn{double n1n2prod = n1*n2;}\\
    \ \ \ \ 3 & \CodeIn{final int n1n2prod =2*( n1+ n2+1);}\\
    \ \ \ \ 4 & \CodeIn{double n1n2prod = n2*( n1+ n2+1) /2.0;}\\
    \ \ \ \ 5 & \CodeIn{final double n1n2prod = n1*( n1+2+1) /2.0;}\\
    $\star$ 6 & \CodeIn{final double n1n2prod = n1*n2;}\\
      & ...  \\
    \ \ \ 33 & \CodeIn{int n1n2prod = n1*2*2;} \\
    \bottomrule
  \end{tabular}%
  }
% \vspace{-2ex}
 
  
\end{table}


Now, Alice needs to sift through these 33 patches to identify the correct one. This is tedious and time-consuming, especially given that many patches look very similar to each other and only have subtle differences. To fully understand why each patch fixes the test failure, Alice needs to manually debug the patch and examine its runtime behavior. Though she may not have to debug all 33 plausible patches, only debugging several promising ones may already take a long time, since she can only debug one patch at a time. Specifically, she not only has to set breakpoints and step through each patch but also examine the runtime behavior difference among different patches. This is cognitively demanding---she has to remember the runtime values of the previous patch, then compare them with the runtime values of the current patch, and repeat until she finds the correct patch. 

\iFix is designed to reduce the cognitive load of examining and selecting patches generated by APR tools. Given a set of plausible patches, \iFix  first runs a multi-criteria clustering algorithm to select a small yet diverse set of representative patches, as shown in Table \ref{table:ifix-picked-patches}. In this way, Alice will not be overloaded with a large number of patches at the beginning. If Alice finds a promising patch from the shortlist, she can ask \iFix to show additional similar patches to further explore. By contrast, if some patches are obviously wrong, Alice can ask \iFix to filter out similar patches that are also likely to be nonsensical. In addition, \iFix provides a holistic behavior comparison table to help Alice examine the runtime behavior difference between patches in one glance. \iFix runs individual patches one by one at the back end, logs the runtime values of variables and expressions related to the patch, and aligns and renders the runtime values in a comparison table, as shown in Table \ref{table: example-runtime}.

\begin{table}[h]
\small
  {%
  % \vspace{-2ex}
  \caption{Four patches selected and ranked by \iFix.}
  \label{table:ifix-picked-patches}
  %\vspace{-2ex}
  \begin{tabular}{cc}
    \toprule
    Index & \iFix-selected Patches\\
    \midrule
    $\star$ 1 & \CodeIn{final double n1n2prod = n1*n2;}\\
    \ \ \ \ 2 & \CodeIn{double n1n2prod = n2*( n1+ n2+1) /2.0;}\\
    \ \ \ \ 3 & \CodeIn{double n1n2prod = n1*( n2+ n2) /2.0;}\\
    \ \ \ \ 4 & \CodeIn{final int n1n2prod =2*( n1+ n2+1);}\\
    \bottomrule
  \end{tabular}%
  }
  % \vspace{-2ex}
  
  
\end{table}


 After examining the runtime values, Alice notices a significant difference in the return values of  \CodeIn{FastMath.sqrt(VarU)} between the buggy code and all plausible patches. In the buggy code, its value is \CodeIn{NaN}, while the value in all patches is a real number. Further analysis of the runtime values of the variable \CodeIn{VarU} reveals that it is a negative number in the buggy code, whereas it is a positive number in  all patches. Since negative numbers do not have a square root, Alice now figures out that the \CodeIn{NaN} in the buggy code is caused by this negative number. Based on Line\#177 in Figure~\ref{fig:codebase-1}, \CodeIn{VarU} is computed from \CodeIn{n1n2prod * (n1 + n2 + 1) / 12.0}. Given that \CodeIn{n1n2prod}, \CodeIn{n1}, and \CodeIn{n2} are all positive numbers in Table ~\ref{table: example-runtime}, \CodeIn{VarU} is supposed to be positive as well, theoretically. Then, Alice notices that the runtime values of \CodeIn{n1n2prod}, \CodeIn{n1}, and \CodeIn{n2} are very big. She realizes that an integer overflow occurs when computing \CodeIn{VarU}, which leads to a negative value. She needs to use a different data type rather than \CodeIn{int}, which is only 4 bytes in Java (maximum value is $2147483647$). 


\begin{table*}
% \small
\caption{Behavior Comparison of the Buggy Method \CodeIn{calculateAsymptoticPValue} in Figure \ref{fig:codebase-1}}
  %\vspace{-2ex}
  \label{table: example-runtime}
  \resizebox{0.7\textwidth}{!}{%
   
  \begin{tabular}{l|rrrrr}
    \toprule
    \multicolumn{1}{c|}{Runtime Variables} & \multicolumn{1}{c}{\multirow{1}{*}{{Buggy}}} & \multicolumn{1}{c}{{\multirow{1}{*}{Patch 1}}} & \multicolumn{1}{c}{{\multirow{1}{*}{Patch 2}}} & \multicolumn{1}{c}{{\multirow{1}{*}{Patch 3}}} & \multicolumn{1}{c}{{\multirow{1}{*}{Patch 4}}}\\
    % \multicolumn{1}{c|}{Variables} & & & & \\
    \midrule
    
    \CodeIn{n1} & 1500 & 1500 & 1500 & 1500 & 1500\\
    \CodeIn{n2} & 1500 & 1500 & 1500 & 1500 & 1500\\
    \CodeIn{n1n2prod} & \cellcolor{red!10} 2250000 & \cellcolor{green_b!35} 2250000.0 & \cellcolor{green_c!35} 2250750.0 & \cellcolor{green_b!35} 2250000.0 & \cellcolor{green_d!35} 6002\\
    \CodeIn{EU} & \cellcolor{red!10} 1125000.0 & \cellcolor{green_a!35} 1125000.0 & \cellcolor{green_b!35} 1125375.0 & \cellcolor{green_a!35} 1125000.0 & \cellcolor{green_c!35} 3001.0\\
    \CodeIn{VarU} & \cellcolor{red!10} -153140382.667 & \cellcolor{green_b!35} 562687500.0 & \cellcolor{green_c!35} 562875062.5 & \cellcolor{green_b!35} 562687500.0 & \cellcolor{green_d!35} 1501000.167\\
    \CodeIn{FastMath.sqrt(VarU)} & \cellcolor{red!10} \HighlightInRed{NaN} & \cellcolor{green_b!35} 23721.035 & \cellcolor{green_c!35} 23724.988 & \cellcolor{green_b!35} 23721.035 & \cellcolor{green_d!35} 1225.153 \\
    \CodeIn{z} & \cellcolor{red!10} \HighlightInRed{NaN} & \cellcolor{green_b!35} -0.032 & \cellcolor{green_c!35} -0.047 & \cellcolor{green_b!35} -0.0312 & \cellcolor{green_d!35} 915.191 \\
    \CodeIn{cumulativeProbability(z)} & \cellcolor{red!10} {\HighlightInRed{NaN}} & \cellcolor{green_b!35} {0.487} & \cellcolor{green_c!35} {0.481} & \cellcolor{green_b!35} {0.487} & \cellcolor{green_d!35} {1.0} \\   
    \bottomrule
  \end{tabular}%
  }
 
\end{table*}

After examining the runtime values of the buggy method when applied with the 4 candidate patches, Alice takes a closer look at the candidate patches themselves. She observes that Patch 1 differs from the other patches in that it only changes the type of the variable \CodeIn{n1n2prod}, while the other patches change the expression on the right-hand side. Based on her understanding of the root cause of the bug, Alice considers Patch 1 to be the most promising among the candidates. With the help of \iFix, she is able to quickly select this patch as the correct one among those generated by Automatic Program Repair tools. Alice is also confident in her selection as \iFix has helped her identify the root cause of the bug.




==> templates/3-Methodology.tex <==
% \todo{you should describe \iFix as a APR-agnostic tool. It doesn't rely on CURE. CURE can be one backend APR tool but it can also be other APR tools. Don't even mention CURE here.}The IPR framework is based on the result of CURE (and will be able to support multiple APR tools) and contains three main components: 1) the sampling and clustering \todo{don't use a term like "back-end server" here. it makes your approach section sounds very engineering.}back-end server, 2) the program instrument back-end server, and 3) a VS Code extension which works as the front-end and manages the interaction between user and back-end servers. Figure \ref{fig:ipr-framework} demonstrates the main architecture and the data flow of IPR.

% \iFix provides a novel integration of hierarchical clustering, code static analysis and code instrument techniques to help improve the usability of APR tools and build trust between APR-generated patches and the developers. To make it possible, we first proposed Multi-Criteria-Based Patch Sampling to reduce the workload of investigating hundreds of APR-generated patches. Second, our Runtime Behavior Comparison approach helps developers understand the root cause of the bug and the differences among the patches without manually debugging the program step-by-step.

\iFix is designed to facilitate the patch comprehension, validation, and selection process of using APR tools. Given a set of auto-generated patches, it selects a small yet diverse subset of patches and computes the behavior difference among these patches.  %is an innovative integration of hierarchical clustering, code analysis and code instrumentation techniques that aims to enhance the usability of automated program repair (APR) tools and build trust in APR-generated patches among developers. 
\iFix includes two key components: (1) {\em multi-criteria patch sampling and re-ranking} (Section~\ref{subsec:multi-criteria}) and {\em Runtime Behavior Comparison} (Section~\ref{subsec:comparison}). The first component reduces the workload of examining many APR-generated patches, while the second component enables developers to understand the root cause of the bug and distinguish patches without having to manually debug the program in a step-by-step manner. We explain each of them below. %Overall, \iFix presents a promising solution to pipeline the APR process and facilitate effective collaboration between developers and APR tools.


\subsection{Multi-criteria Patch Sampling \& Re-ranking}
\label{subsec:multi-criteria}
Previous studies have shown that APR tools~\cite{jiang_cure_2021, chen_sequencer_2019, lutellier_coconut_2020, xia_less_2022, liu2019tbar} can automatically generate a large set of {\em plausible patches} that pass the previously failed test cases but are not necessarily correct~\cite{smith_is_2015, le_overfitting_2018}. It is tedious and time-consuming to manually inspect those patches, understand their differences, and select the correct one. Inspired by the literature of active learning~\cite{settles2009active}, we propose a novel multi-criteria patch sampling method. The key insight is to iteratively sample a small set of patches that are {\em diverse} and {\em representative}, so developers can interactively examine a small number of patches each time, provide feedback, and gradually narrow down to the correct one in a large patch space. %The sampled patches are further ranked based on the \textit{similarity} between each patch and the original buggy code. 
Algorithm \ref{algorithm: multi-criteria} describes the multi-criteria patch sampling process.
%\vspace{-1ex}
\begin{algorithm}[]
\caption{Multi-Criteria Patch Sampling \& Re-ranking}
\label{algorithm: multi-criteria}
\small
\DontPrintSemicolon
  
  \KwInput{Plausible Patch List $ P $, Target Buggy Code $ B $}
  \KwOutput{Sampled Patch List $ L $}
  
  $ UL \leftarrow \{\}  $
  
  %\If{length(P) > 10}
  %{
    $ C \leftarrow Hierarchical\_Cluster(P) $

    \For{$ c $ in $ C $}
    {
      $ centroid \leftarrow Select\_Centroid(c)$
    
      $ UL.append(centroid)  $
    }
  %}
  
  %\Else
  %{
  %	$ UL \leftarrow P  $
  %}
  
  $ L \leftarrow Rank\_By\_Similarity(UL, B) $


\end{algorithm}


A diverse set of patches may give developers hints on how to fix a bug from different perspectives. To select diverse patches, \iFix first uses a hierarchical clustering algorithm~\cite{Hierarchical} to cluster the given patches based on their similarity (Line 2 in Algorithm \ref{algorithm: multi-criteria}). Compared with other clustering algorithms such as K-Means~\cite{K-means} and KNN~\cite{KNN}, hierarchical clustering is not sensitive to initialization conditions such as the random seeds and the original ranking. Furthermore, compared with K-Means and KNN, there is no need to specify the number of clusters beforehand. %It also provides detailed information about which patches are most similar to each other. 
We use Levenshtein distance~\cite{levenshtain} between the tokenized patches as the similarity metric for clustering. %, which is denoted as $ LV\_Dist(p_i, p_j) $.  The similarity between the tokenized patches is then defined as $ LV\_Sim(p_i, p_j) = 1 - LV\_Dist(p_i, p_j) $. Based on this similarity metric, \iFix clusters plausible patches into several clusters, thus ensuring the diversity criterion.
After the clustering process, \iFix selects the most representative patch from each cluster (Line 4 in Algorithm \ref{algorithm: multi-criteria}). The representativeness of a patch can be evaluated based on how many patches are similar to it in a cluster. Given a patch cluster $ C = \{ p_1, p_2, ... , p_n \} $, for each patch $ p_i $, its representativeness is defined in Equation \ref{equation: representativeness}: 

\begin{equation}
\label{equation: representativeness}
    R (p_i) = \frac{\sum_{j \neq i} Levenshtein\_Distance(p_i, p_j)}{n - 1}
\end{equation}


 \iFix selects the patch with the largest $ R $ from each cluster. This is also 
equivalent to selecting the centroid of each cluster, which can be seen as the most representative patch in a cluster.

Finally, \iFix ranks the representative patches selected in the previous step to increase the chance that developers see the correct patch as early as possible (Line 6 in Algorithm \ref{algorithm: multi-criteria}). Our ranking heuristic is based on an insight that has been observed in several prior work~\cite{d2016qlose, le2017s3, wen2018context, wang2020automated}---{\em a correct patch is more likely to be similar to the buggy code}. 
For each selected patch, \iFix tokenizes it and calculates its Levenshtein distance to the tokenized buggy code and ranks them based on the Levenshtein distance. 

% Based on the multi-criteria-based patch sampling process, \iFix selects the centroid of each cluster, which ensures the representativeness of the final sampled list; the selected patches are from different clusters, which can be considered diverse to each other; the ranking procedure ensures that the correct patch will be more likely to be put in the front of the shown list. Note that if the number of plausible patches generated by the APR tool for one bug is less than 10, \iFix will directly rank all the plausible patches without clustering and sampling.


\subsection{Runtime Behavior Comparison}
\label{subsec:comparison}
% We proposed a runtime behavior comparison approach to provide a real-time view of run-time information of a bunch of patches to the user. The module collaborates with the Multi- Criteria ranking algorithm to assist the user in selecting the most favorable patch \todo{among what?}.

% The goal of the Runtime Behavior Comparison approach is to provide full debug information so as to eliminate the potential debugging efforts of the developers. To make it possible, \iFix first copy the project directory including the buggy program, each applied with one of the candidate patches. \iFix then employs static analysis and make code instrument in the source code to log runtime values. Finally, \iFix runs the failed test case on the projects in parallel and collects the output of the log statements instrumented in the previous step.

The primary objective of this component is to provide developers with comprehensive debugging information for them to understand and validate auto-generated patches. 
\iFix achieves this in three steps. Since the execution trace of a test failure contains many method invocations and runtime values, \iFix first performs call graph analysis and def-use analysis to identify a small set of runtime values related to the failure-inducing statement in the execution trace of the failed test case. Then, \iFix performs code instrumentation to log the related runtime values. Finally, \iFix analyzes the logged values and aligns them across different patches for easy comparison. We elaborate each step below.

% Inspired by the idea of differential testing~\cite{journals/dtj/McKeeman98}, we designed a component to help display the run-time values of significant variables in the stack traces that indicate how the bug is triggered. Based on an existing java program analysis framework~\cite{zhang_grafter_2018}, we developed a program to make instrumentation inside the code, which helps log the values of significant variables and sub-expressions. 

\textbf{Call Graph Analysis}.
%\fixed{you need to explain why you need to do call graph analysis. Remember the moment we decided to do this analysis? It's because we realized at that time there is a "gap" between the buggy code and the test case. So we want to show users how the buggy code is invoked by the test case and how the incorrect values computed in the buggy code "flow" towards the assertion statement through the call graph. You need to explain here. Otherwise,your reviewers won't understand why call graph analysis.} 
\iFix performs dynamic analysis to capture the call stack traces during execution. Specifically, \iFix leverages the \CodeIn{java.lang.getStackTrace} API to log the call stack trace of the buggy statement. This logged call stack trace includes the name of a method call in the stack trace, the name of the class where the method is defined, and the line number and file name of the method invocation. For example, the call stack trace of the buggy statement in Figure~\ref{fig:codebase-1} includes the information about  \CodeIn{calculateAsymptoticPValues}, \CodeIn{mannWhiteneyUTest}, and \CodeIn{testBigDataSet}. The call stack trace will not only help us narrow down the scope of def-use analysis in the next step but also helps developers understand how the buggy statement is triggered by the test case as well as how the faulty values propagate through the stack trace to the failure. 

% To achieve this, \iFix makes use of the \CodeIn{getStackTrace()} method from the \CodeIn{java.lang} library's \CodeIn{Throwable} class, which provides essential interfaces that handle errors and exceptions. \iFix instruments code snippets before the buggy code to extract and log the stack trace information. This information consists of several entries. Each entry contains the name of a method $M$ in the stack trace, the name of the class and file where the method is defined, and the entry line number $N$ where it calls the previous method in the stack trace. For the top method in the stack trace, $N$ indicates the line number of the buggy code. \iFix makes use of the class and file names to locate the corresponding files in the implementation.

% \begin{table*}[hbtp]
%   % \resizebox{\columnwidth}{!}
%   {%
%   \begin{tabular}{c|ll|ll}
%     \toprule
%      & \multicolumn{2}{c|}{{Stack Trace}} & \multicolumn{2}{c}{{Runtime Variables}} \\
%      \midrule
%      \multirow{4}{*}{1} & \CodeIn{Method:} & \CodeIn{calculateAsymptoticPValue} & \CodeIn{Variable:} & \CodeIn{n1, n2, n1n2prod, Umin, EU, VarU, z}\\
%      & \CodeIn{Class:} & \CodeIn{MannWhitneyUTest} & \CodeIn{MethodCall:} & \CodeIn{FastMath.sqrt(VarU),  NormalDistribution(0, 1)}\\
%      & \CodeIn{File:} & \CodeIn{MannWhitneyUTest.java} & \CodeIn{} & \CodeIn{standardNormal.cumulativeProbability(z)}\\
%      & \CodeIn{Line:} & \CodeIn{175} & \CodeIn{Expression:} & \CodeIn{n1 * n2, n1n2prod / 2.0, ...}\\
%      \hline
%      \multirow{4}{*}{2} & \CodeIn{Method:} & \CodeIn{mannWhitneyUTest} & \CodeIn{Variable:} & \CodeIn{Umin}\\
%      & \CodeIn{Class:} & \CodeIn{MannWhitneyUTest} & \CodeIn{MethodCall:} & \CodeIn{calculateAsymptoticPValue(Umin, x.length, y.length)}\\
%      & \CodeIn{File:} & \CodeIn{MannWhitneyUTest.java} & \CodeIn{Expression:} & \CodeIn{-}\\
%      & \CodeIn{Line:} & \CodeIn{237}\\
%      \hline
%      \multirow{4}{*}{3} & \CodeIn{Method:} & \CodeIn{testBigDataSet} & \CodeIn{Variable:} & \CodeIn{result, d1, d2}\\
%      & \CodeIn{Class:} & \CodeIn{MannWhitneyUTestTest} & \CodeIn{MethodCall:} & \CodeIn{testStatistic.mannWhitneyUTest(d1, d2)}\\
%      & \CodeIn{File:} & \CodeIn{MannWhitneyUTestTest.java} & \CodeIn{Expression:} & \CodeIn{-}\\
%      & \CodeIn{Line:} & \CodeIn{112}\\
%     \bottomrule
%   \end{tabular}%
%   }
%   \caption{Stack Trace and Runtime Variables Extracted from Code Snippets in Figure \ref{fig:codebase-1}}
%   \label{tab:code-analysis-res}
%   \vspace{-2ex}
% \end{table*}







% \iFix employs call graph analysis to identify the callers of the buggy program. This results in a tree in which each node represents a method invoked by its parent. By traversing this tree, our component returns a list of traces ending at the buggy method.

\textbf{Def-Use Analysis}. Based on the call graph analysis result, \iFix performs def-use analysis on each method in the stack trace of the buggy statement. Since there are many variables in each method, it would be overwhelming if \iFix renders all of them to developers. Thus, this step aims to identify the variables related to the faulty value produced from the buggy statement in each method. %Such approach extracts the runtime variables that exhibit correlation to the propagation of the buggy code during the execution of the test case. 
A variable is considered {\em defined} if it is assigned a new value, e.g., appearing on the left-hand side of an assignment statement. A variable is considered {\em used} if its value is used to compute another value in an expression. Def-use analysis will return {\em def-use chains} for all variables defined in a method, as well as {\em use-def chains} for all variables used in a method. A def-use chain of a variable consists of the definition of the variable and all of its use locations reachable from that definition without any other intervening definitions. For example, the defined variable in the buggy statement in Figure~\ref{fig:codebase-1} is \CodeIn{n1n2prod}. Its use locations include Line 176 and Line 177. By contrast, a use-def of a variable consists of a location that uses the variable and all the variables that are directly computed from that variable in that location.

Algorithm~\ref{algorithm: def-use} describes the procedure to gather runtime values affected by the buggy statement based on def-use analysis. After def-use analysis (Line 1), \iFix first identifies the variable {\em defined} by the buggy statement (Line 2). Then, it analyzes the def-use chains ($DU\_Chain$) of these variables and identifies all their used locations (Line 7). Given the use locations, it further analyzes the use-def chains ($UD\_Chain$) to identify the variables defined in those locations with the values computed from the buggy statement. For example, in Figure~\ref{fig:codebase-1}, from the two use locations (Line 176 and Line 177) of the faulty value in \CodeIn{n1n2prod}, \iFix identifies that \CodeIn{VarU} and \CodeIn{z} are further computed from the faulty value in these two locations. \iFix  repeats this step until no new variables are found (Lines 4-10). In this way, \iFix captures the propagation of a faulty value in a method. To continue tracing the propagation of the faulty values in the caller of the buggy method, \iFix runs the same procedure in Algorithm~\ref{algorithm: def-use} on the method invocation statement and continues to process other methods in the call stack. For example, in Figure~\ref{fig:codebase-1}, \iFix analyzes the variables by the call site at Line 231 in \CodeIn{calculateAsymptoticPValue}, and further analyzes the variables by the call site at Line 113 in \CodeIn{mannWhiteneyUTest}.

%\vspace{-2ex}
\begin{algorithm}[h]

\DontPrintSemicolon
\caption{Identify variables affected by a statement}
\label{algorithm: def-use}


\small
  % \KwInput{Method $M$, Line Number of Invocation $N$}
  \KwInput{Statement $s$, Method $m$}
  \KwOutput{Variables affected by the statement $s$}
  
  % $ RV \leftarrow \{\}  $
  
  % $ Y \leftarrow  Get\_Last\_Line\_Number(M) $
  
  % $ RV.append(Def(M, N, Y) \cup Use(M, N, Y)) $
  
  % $ RV.append(MethodCalls(M, N, Y)) $
  
  % $ RV.append(SubExpression(M, N, Y)) $

  $DU\_Chains, UD\_Chains \gets Def\_Use\_Analysis{(m)}$ 

  $d \gets {Get\_Defined\_Variable}{(s, DU\_Chains)}$  

  $D.\text{append}(d)$

  $R \gets \{\}$
      
  % $newVarsFound \gets \text{true}$
  
  \While{$D \neq \varnothing$}
    % {$newVarsFound \gets \text{false}$
    {$v \gets D.\text{pop}()$
    
    $R.\text{append}(v)$
    
    \For{$u \in DU\_Chains.\text{get}(v)$}
      {$D.\text{append}({UD\_Chains}.\text{get}(u))$
      
      $R \gets R.append(u)$
      
      }}
  $R \gets R \cup {DU\_Chains}.\text{get}(d)$
  
  \textbf{return} $R$
\end{algorithm}
%\vspace{-2ex}
% Given a method $M$ and its entry line number $N$, the runtime variables $RV$ logged by \iFix can be approximated:

% \begin{displaymath}
% \begin{split}
% Y &= \mathrm{Get\_End\_Index}(M) \\
% Variable &= \mathrm{Def}(M, N, Y) \cup \mathrm{Use}(M, N, Y) \\
% MethodCall &= \mathrm{Method}(M, N, Y) \\
% Expression &= \mathrm{Expr}(M, N, Y) \\
% RV &= \{Variable, MethodCall, Expression\}
% \end{split}
% \end{displaymath}

% To extract runtime variables using def-use analysis, \iFix introduced an Abstract Syntax Tree (AST) visitor that includes essential functions. $\mathrm{Def}(M, X, Y)$ returns $(v, l)$ pairs, in which $v$ indicates variables declared in method $M$ within a range of line number $(X, Y)$, and $l$ indicates the line number where $v$ is declared. Similarly, $\mathrm{Use}(M, X, Y)$, $\mathrm{Method}(M, X, Y)$ and $\mathrm{Expr}(M, X, Y)$ return the used variables, the method calls and the sub-expressions in method $M$ between line $X$ and $Y$ along with the exact line numbers. $\mathrm{Get\_End\_Index}(M)$ returns the line index of the end of function $M$. To gather the necessary runtime information in the stack trace, \iFix selects the defined variables, method calls and sub-expressions occur in the methods after the entry line, as well as the used variables not defined within that range. \iFix also logs the exact line number of each runtime variable.

% Table \ref{tab:code-analysis-res} illustrates the result of code analysis on the example code snippets shown in Section \ref{sec:MotivatingExample}.

% \iFix performs def-use analysis to identify variables that are related to the buggy line. \todo{You need to first formally define what you mean by related as I did in my ICSE 2017 paper and then illustrate it with a Figure.} Figure 4 illustrates this idea. In this figure, the buggy line is indicated \todo{indicated by what?} and all code that is potentially affected by the buggy line is colored in yellow. \todo{I don't understand the following sentence. If you find related variables based on def and use, why some of them contain irrelevant information?}Although the related code contains all the information that users might be interested in, it also includes irrelevant information: in a block of "related" code, not every line of code is affected by the buggy line.\todo{specify which variable contains irrelevant information in the figure} To provide more concise but equally useful information, \iFix applies two rules that further select information from "related" code. \todo{Isn't this the definition of related variables/expressions?}The first rule is to select code that uses the variable(s) that is used in the buggy line, and the second rule is to select code that uses  variables that are defined by the variable(s) used in the buggy line. In this way, \iFix only provides bug-related information to users. 


\textbf{Code Instrumentation} Given the related variables identified from the previous step, \iFix instruments the defined and used locations of these variables to log their runtime values. \iFix utilizes the {\em XStream} library~\cite{noauthor_xstream_nodate} in Java to serialize the runtime values of those variables as well as their locations into an XML file. %These XML strings, along with the name, type, and line number of the runtime values, are then written to temporary files with file-writing statements, which are subsequently instrumented into the code base. 
In addition to logging those variables, \iFix also logs the runtime values of method calls and subexpressions that use the identified variables since developers may also wonder their runtime values during debugging. For example, in Figure~\ref{fig:codebase-1}, \iFix logs the value of \CodeIn{n1+n2+1} in Line 177 and the value of \CodeIn{FastMath.sqrt(VarU)} in Line 179. 

%In addition to performing code instrumentation on the original version of the buggy code, \iFix applies each candidate patch suggested by {\em multi-criteria patch sampling and re-ranking} (described in Section \ref{subsec:multi-criteria}) and conducts instrumentation concurrently. \iFix compiles these instrumented code bases and runs the failed test case on them. Finally, \iFix gathers the files that contain the outputs generated by the instrumented statements and feeds them into the UI widget (Section \ref{sec:UserInterface}) for visualization.

% \Comment{\textit{Illustrating iterative and recursive calls.}
Finally, \iFix analyzes the log files and aligns the runtime values based on their locations between the buggy code and  different patches. In this alignment process, a special case is the runtime values logged from a variable in a loop or a method called multiple times during the test execution. In such cases, the log files will contain multiple runtime values for the variable in the same location. For example, in Figure~\ref{fig:codebase-2}, the variable, \CodeIn{pos}, will be logged multiple times in the loop. Furthermore, the number of the logged values of the same variable may vary across different patches since the patches may alter the loop iterations differently. To handle such cases, \iFix assigns an index to each runtime value of the same variable logged in the same location based on their appearance in the log files. Then, it aligns these values based on the indices. For runtime values that are logged many times across iterations, \iFix identifies the iteration where the behavioral divergence occurs for the first time (i.e., the runtime values of the same variable differ from the buggy code and the patch) and renders the runtime values at that iteration to developers to avoid overwhelming them.
%In situations where there are loops or repeated calls to the same method, the value of a runtime variable may vary across different iterations. If its value is simply updated within the same row in the table, users may miss important information regarding to the root cause of the bug. For example, in another bug Lang 6 which belongs to Defects4J, the behavior of runtime values vary in a \CodeIn{for} loop, as shown in Table \ref{tab:example-runtime-2}. Notice that as the 2nd argument of the method \CodeIn{Character.codePointAt} varies among the buggy code and patches, it is important for the \iFix to ensure that users can still identify and compare these different method calls during the program's execution.

{\begin{figure}[hbtp]
\vspace{4pt}
\begin{lstlisting}[language=Java, firstnumber=94]
for (int pt = 0; pt < consumed; pt++) {
    pos += Character.charCount(Character.codePointAt(input, pos));            /* Buggy */
//  pos += Character.charCount(Character.codePointAt(input, 0));              /* Patch 1 */
//  pos += Character.charCount(Character.codePointAt(input, pt));             /* Patch 2 */
}\end{lstlisting}
\caption{A buggy statement in a loop (Lang 6 in Defects4J)}
\label{fig:codebase-2}
\end{figure}}





% \todo{the first sentence is too low-level}\iFix creates multiple threads to run in parallel, each with the buggy line replaced with a certain patch generated by \todo{don't mention CURE.}CURE. \todo{you should mention you used XStream to log runtime values.}Our component parses the original Java files and inserts log statements into the Java files. \todo{You should explain how you insert counters in the log statement to handle loops and multiple invocations.}%Where these log Statements are inserted are determined by the line number information Instrument acquires when accomplishing the first goal.

% At last, our component runs the test method to execute the programs along with the inserted log statements so that run-time values are logged and ready to be displayed to our user. It then displays all the variables and expressions that the developer may concern about in an all-in-one table, namely the Function Behavior Table.  
    
% To achieve this task, the first goal is to identify the stack traces and the significant variables in the stack traces. First, {\tool} applies call graph analysis to identify the callers of the buggy program. This results in a tree in which each node represents a method invoked by its parent. By traversing this tree, our component returns a list of traces ending at the buggy method. Second, {\tool} performs def-use analysis to identify variables that are closely "related" to the buggy line. The definition of "related" can be properly explained in Figure 4: in this example, the buggy line is indicated and all code that is potentially affected by the buggy line is colored in yellow. Although the "related" code contains all the information that users might be interested in, it also includes irrelevant information: in a block of "related" code, not every line of code is affected by the buggy line. To provide more concise but equally useful information, {\tool} applies two rules that further select information from "related" code. The first rule is to select code that uses the variable(s) that is used in the buggy line, and the second rule is to select code that uses  variables that are defined by the variable(s) used in the buggy line. In this way, {\tool} only provides bug-related information to users. 

% When our component acquires the variable information and the stack traces, the next thing it does is to instrument the buggy program. {\tool} creates multiple threads to run in parallel, each with the buggy line replaced with a certain patch generated by CURE. Our component parses the original Java files into lists of Strings based on their system eliminators and inserts log Statements into the Java files. Where these log Statements are inserted are determined by the line number information Instrument acquires when accomplishing the first goal. At last, our component runs the test method to execute the programs along with the inserted log Statements so that run-time values are logged and ready to be displayed to our user. It then displays all the variables and expressions that the developer may concern about in an all-in-one table, namely the Function Behavior Table.  



==> templates/4-UserInterface.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{./Figures/ui-overview.pdf}
    % \precaptionspace
    %\vspace{-2ex}
    \caption{The User Interface of \iFix}
    % \vspace{-2ex}
    \label{fig:ui-overview}
\end{figure*}

We develop a VS Code extension as the front-end interface for \iFix. Figure \ref{fig:ui-overview} gives an overview of the user interface. Our interface includes three major features: {\em Interactive Patch Exploration}, {\em Behavior Comparison Table}, and {\em Navigation Support}. 
    
% \textbf{Interactive Patch View} 
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{./Figures/ifix-patchview.png}
%     % \precaptionspace
%     \caption{The Interactive Patch View of \iFix}
%     \vspace{-2ex}
%     \label{fig:ifix-patchview}
% \end{figure}

% The \iFix extension displays patch by cluster in the main text editor where the original code with buggy line is edited and decorated. User can control the process of sampling as well as clustering by clicking the button 'explore the cluster', 'exclude the cluster', 'accept patch', etc.

\textbf{Interactive Patch Exploration \xspace} 
%The Interactive Patch View displays patches based on the result of Multi-Criteria Ranking as explained in Section \ref{subsec:multi-criteria}. 
This feature is built on top of the source code editor in VS Code. It renders the shortlist of representative and diverse patches selected by the multi-criteria sampling algorithm in Section \ref{subsec:multi-criteria}.  For each patch, a user can dive into the cluster of patches it represents by clicking the {\em Explore Similar Patches} button over it. This feature is extremely useful in cases where the initially selected patch looks promising but is not fully correct, since users can explore similar patches in the same cluster and locate the correct one. On the other hand, if a patch looks completely wrong, users can reject it and all other adjacent ones which are likely to be wrong, by clicking the {\em Exclude Similar Patches} button. Using these two interactive features together, the user can easily navigate a large number of patches and quickly locate the patch that looks the most promising to her. %the patch view provides three operations: explore more patches, exclude similar patches and accept patch. \ruixin{@zhongkai, how do we call the patches which does not take representative of a cluster of patches?}
    
% \textbf{Runtime Behavior Table}
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{./Figures/ifix-table.png}
%     % \precaptionspace
%     \caption{The Runtime Behavior Table of \iFix}
%     \vspace{-2ex}
%     \label{fig:ifix-table}
% \end{figure}

\textbf{Behavior Comparison Table \xspace} 
% \iFix provides a table to visualize the data collected in Runtime Behavior Comparison (\ref{subsec:comparison}). 
% To generate such a table, the user clicks on the {\em rerun} button right after the failed test case displayed at the top of the \iFix side bar. The table is located at the bottom of this panel. It displays the differences in runtime variables (including defined or used variables, method calls, and infix expressions) of all methods in the stack trace, from the buggy method to the failed test method. If the user is interested in one of the methods, she can click on the name name of the method to expand it. Otherwise she can click on its name again to collapse. The first column of the table shows the line number at which the runtime variable occurs, and the second column shows the name of the runtime variable. The following column displays its value with the buggy code as well as under the candidate patches.
%To visualize the data collected in Runtime Behavior Comparison (\ref{subsec:comparison}), 
\iFix aligns the runtime values captured for each patch (Section \ref{subsec:comparison}) and renders them in a series of comparison tables. \iFix generates a table for each method in the call stack of the buggy statement, with the first table corresponding to the method in which the buggy statement appears, and the last table corresponding to the test method. The layout of these tables resembles the call stack view in a regular debugger. \iFix adopts this design to help developers comprehend the data flow during the test execution, such as the propagation of the faulty values from the buggy statement to the assertion statement in the test case. %To access this table, the user simply clicks on the "rerun" button located adjacent to the failed test case displayed at the top of the \iFix side bar.
For a test execution trace with many method calls, the user can collapse the comparison tables for those less important methods to simplify the user interface. 

In each behavior comparison table, the first column shows the line number at which the runtime value is logged. The second column shows the name of the runtime value, which can be a variable name, a method call, or a subexpression. The following columns display the runtime value logged from the original buggy code, as well as from individual patches. To help developers easily see the differences in runtime values, \iFix color-codes each unique value in a row. As shown in Figure \ref{fig:ui-overview}, if the buggy code has a different runtime value than the patches, the corresponding cell is rendered in red, while cells with unique values in the patches are rendered in different shades of green. %This color scheme provides a clear visual indicator of the effectiveness of the candidate patches in resolving the bug, allowing developers to quickly identify the most promising solutions.
Furthermore, to reduce the visual clutter of rendering many runtime values, \iFix combines adjacent cells with the same runtime value. For example, the runtime values of \CodeIn{m1} are merged into a single cell in Figure~\ref{fig:ui-overview}. 

\begin{figure}
    \centering
    % \includegraphics[width=\columnwidth]{./Figures/ifix-patchview.png}
    \includegraphics[width=\columnwidth]{./Figures/ifix-table.pdf}
    % \precaptionspace
    %\vspace{-2ex}
    \caption{Output of \iFix for the Bug in Figure \ref{fig:codebase-2}}
    %\vspace{-2ex}
    \label{fig:ui-preview-2}
\end{figure}


Finally, to distinguish runtime values logged from different loop iterations or repeated method calls, \iFix adds the index of the loop iteration or method call after the line number, separated by \#. For subexpressions and method calls that vary across patches, \iFix synthesizes a new name to align their values in a single row. Specifically, \iFix retains the common substrings and substitutes the variations with a wildcard symbol *. For example, in Figure~\ref{fig:codebase-2}, the patches substitute the second argument of \CodeIn{Character.codePointAt} with different values. \iFix synthesizes a new name, \CodeIn{Character.codePointAt( input, *)} to represent this method call, so it can render the return value of this method call from different patches in the same row, as shown in Figure~\ref{fig:ui-preview-2}.




{\bf Navigation Support} If a user wants to investigate the original code where a runtime variable occurs, they can simply click on the variable name within the Runtime Behavior Table. Once the user clicks on the variable name, the text editor will automatically navigate to the corresponding line, allowing the developer to quickly review the code and identify potential issues. Meanwhile, to help users distinguish potential variables redefinitions, the table renders the line number where the runtime variable is defined or used.

% \begin{table}
%   \resizebox{\columnwidth}{!}{%
%   \begin{tabular}{c|c||ccccc}
%     \toprule
%     Iteration & Runtime values & Buggy & Patch 1 & Patch 2 & Patch 3 & Patch 4\\
%     \midrule
%     \multirow{3}{*}{1} & Argument^* & 0 & 0 & 0 & 0 & 0 \\
%                       & Return Value^{**} & 2 & 2 & 2 & 2 & 2 \\
%                       & \CodeIn{pos} & 2 & 2 & 2 & 2 & 2 \\
%     \midrule
%     \multirow{3}{*}{2} & Argument^* & 2 & 0 & 1 & 0 & 0 \\
%                       & Return Value^{**} & \textbackslash & 2 & 1 & 2 & 2 \\
%                       & \CodeIn{pos} & \textbackslash & 4 & 3 & 4 & 4 \\
%     \bottomrule
%   \end{tabular} %
%   }
%   \caption{Behavior Comparison of the Code Snippet in Figure \ref{fig:codebase-2}. *{\em Argument} indicates the 2nd argument of method call \CodeIn{Character.codePointAt}; **{\em Return Value} indicates the return value of method call \CodeIn{Character.charCount}.}
%   \vspace{-2ex}
%   \label{tab:example-runtime-2}
% \end{table}





==> templates/5-QuantitativeExperiment.tex <==



% \begin{table*}[]
% \small
% \caption{The number of the correct patch ranks that win, tie, and lose to other ranking methods\todo{remove columns for ASTDist, ASTCOsim, VariableDist and keep this table in a single column}}
% \label{table: win tie lose of different method}
% \begin{tabular}{l|rrrrrrr}
% \toprule
%      & \multicolumn{1}{l}{CURE} & \multicolumn{1}{l}{ASTDist} & \multicolumn{1}{l}{ASTCosSim} & \multicolumn{1}{l}{VariableDist} & \multicolumn{1}{l}{S3} & \multicolumn{1}{l}{Learning-based} & \multicolumn{1}{l}{Similarity-based} \\ \hline
% WIN  & 11                       & 5                           & 7                             & 6                                & 6                      & 22                      & 4                           \\
% TIE  & 17                       & 22                          & 21                            & 23                               & 24                     & 6                       & 25                          \\
% LOSE & 3                        & 4                           & 3                             & 2                                & 1                      & 3                       & 2                           \\  \bottomrule
% \end{tabular}
% \end{table*}

To evaluate our multi-criteria patch sampling \& re-ranking algorithm, we conducted a quantitative experiment to answer the following two research questions:

\begin{itemize}[leftmargin=10mm]
    \setlength\itemsep{0.5mm}
    \item[\textbf{RQ1}] Compared with other patching ranking methods, how effective is our algorithm in terms of the final rank of the correct patch?
    \item[\textbf{RQ2}] How generalizable is our algorithm when applied to patches generated by different APR techniques?
\end{itemize}

%We demonstrate the effectiveness of the multi-criteria patch sampling \& re-ranking method by comparing its results against the patch ranking results from the APR tool, the static patch ranking technique, and the patch re-ranking results given by the large language model (LLM). We also show the contribution of the multi-criteria patch sampling step by conducting an ablation study. Furthermore, we evaluate our multi-criteria patch sampling \& re-ranking method on three different APR tools to demonstrate its generalization ability.

\subsection{Effectiveness of Patch Ranking}
\subsubsection{Experiment setup} In this experiment, we use CURE~\cite{jiang_cure_2021} as the underlying APR technique. CURE is one of the state-of-art APR techniques which can correctly fix 57 bugs from Defects4J v1.2~\cite{just2014defects4j}. Specifically, CURE adopts a deep learning (DL) model that leverages a neural machine translation architecture trained on program repair datasets and augments it with a code-aware search strategy for patch generation. For the sake of sampling and re-ranking, we focus on 31 bugs for which CURE can generate multiple plausible patches with at least one correct one. For each bug, we apply our sampling and re-ranking method and the baselines to those patches generated by CURE and compare the final ranking of the correct patch generated by each method. Our experiment is conducted on a server with Ubuntu 18.04 LTS, an 8-core 3.50 GHz Intel x86-64 CPU, 32 GB RAM, and an RTX A5000 GPU.

\subsubsection{Comparison Baselines}
We select four different kinds of patch ranking methods as our baselines: (1) the original patch ranking given by the APR tool, (2) a state-of-the-art static patch ranking method~\cite{le2017s3}, (3) a learning-based re-ranking method adopted by a state-of-the-art APR tool, AlphaRepair~\cite{xia_less_2022}, and (4) a similarity-based re-ranking method obtained from ablating the multi-criteria clustering step from our approach.   We elaborate on each comparison baseline below. 

\begin{itemize}[leftmargin=*]
    \item \textbf{Original Patch Ranking}: We use the default ranking obtained from CURE~\cite{jiang_cure_2021}. Specifically, CURE ranks patches based on the probability score assigned to each patch by the DL model.

    \item \textbf{Static Patch Ranking}: According to a recent comparative study on static patch ranking methods~\cite{wang2020automated}, S3~\cite{le2017s3}  achieves the best performance in ranking correct patches compared with other static methods proposed in~\cite{wen2018context, xin2017leveraging, tan2016anti}. Therefore, we use S3 as the static patch ranking baseline. Specifically, S3 uses three static code features: {\em Abstract Syntax Tree (AST)-level edit distance}, {\em cosine similarity computed from ASTs}, and {\em the locality of variables and constants}. %, which are denoted as {\em ASTDist}, {\em ASTCosSim}, and {\em VariableDist}, respectively. %ASTDist calculates the number of AST node changes between the patch and the buggy code; ASTCosSim calculates one minus the cosine distance between the vectors representing the occurrences of distinct AST node types of the patch and the buggy code; VariableDist measures the Hamming distance between the vectors representing the locations of variables and constants in expressions of patches and the buggy code. In this experiment, we not only compared with S3 but also compared with ranking with  individual static code features in S3 to understand the contribution of each feature to the ranking results.
    \item \textbf{Learning-based Patch Re-ranking}: A recent APR technique, AlphaRepair~\cite{xia_less_2022}, adopts a pre-trained large language model, CodeBERT~\cite{feng2020codebert}, to rank patches. Specifically, it masks tokens in a patch and uses CodeBERT to predict the probability of the masked token. Then, it uses the average probability of all tokens as the ranking score.
    \item \textbf{Similarity-based Patch Re-ranking}: We create a variant of our algorithm by ablating the multi-criteria clustering step to understand the contribution of our multi-criteria clustering step. For each plausible patch, this variant only calculates the Levenshtein distance to the target buggy code and ranks the patches based on the Levenshtein distance.
     
\end{itemize}




\subsubsection{Evaluation Results}
Table~\ref{table: comparison results of patch ranking} shows the comparison results. Overall, our multi-criteria method outperforms all comparison baselines, with an average ranking position of 1.7 and a median ranking position of 1. %We also calculate the number of bugs where our multi-criteria method wins, ties, and loses to other ranking methods in terms of the final rank of the correct patch, as shown in Table~\ref{table: win tie lose of different method}. 
The results show that our multi-criteria method performs best, following the similarity-based ranking and S3 ranking, while the performance of the learning-based ranking is the worst. 
The multi-criteria clustering \& sampling step improves the overall ranking of correct patches by 22\% compared to the similarity-based method, showing its significant contribution to final results.
Compared to the static code features used by S3, the Levenshtein distance metric turns out to be more effective in ranking correct patches.

\begin{table}[t]
\small
\caption{Comparison of different patch ranking methods}
\label{table: comparison results of patch ranking}
%\vspace{-2ex}
\begin{tabular}{l|rrrrr}
 \toprule
       & \multicolumn{1}{l}{CURE} & \multicolumn{1}{l}{S3} & \multicolumn{1}{l}{Learning-based} & \multicolumn{1}{l}{Similarity-based} & \multicolumn{1}{l}{{\bf \iFix}} \\ \hline
MEDIAN    & 1                                                        & 1                      & 6                       & 1                           & {\bf 1}                        \\
MEAN & 3.5                              & 3.1                    & 25.9                    & 2.2                         & {\bf 1.7}                      \\  \bottomrule
\end{tabular}
\end{table}

% The success of our multi-criteria method can be attributed to two factors. First, our method clusters similar patches and samples the most representative patch from each cluster. This step ensures the diversity of the final patch ranking list and excludes overfitting patches that are similar to the correct patch. Second, the Levenshtein Distance metric measures the cost of inserting, deleting, and updating from the original buggy code to the patch on syntax level, which is more effective in prioritizing correct patches over overfitting patches.

\subsection{Generalizability to Other APR Techniques}
To demonstrate the generalizability of our method, we applied it to patches generated by two other APR techniques,  RewardRepair~\cite{rewardrepair} and KNOD~\cite{knod}, in addition to  CURE~\cite{jiang_cure_2021}. Both RewardRepair and KNOD are recent, open-sourced, and state-of-the-art APR techniques. Specifically, RewardRepair uses a transformer-based~\cite{transformer} architecture and incorporates execution information into the loss function for generating more compilable and correct patches~\cite{rewardrepair}. KNOD uses a new tree decoder to generate  ASTs instead of  source code~\cite{knod}. % , and it further performs domain knowledge distillation to increase the syntactical and semantical correctness of patches~\cite{knod}.\nan{added description of RewardRepair and KNOD} 
Similar to the previous experiment, we use Defects4J~\cite{just2014defects4j} as the benchmark and focus on  bugs for which these APR techniques generate multiple plausible patches with at least one correct patch. We finally obtain 27 bugs for RewardRepair, 31 bugs for CURE, and 44 bugs for KNOD.

\begin{table}[t]
\small
\caption{Effectiveness of our method on different APR tools}
\label{table: comparison results of APR}
%\vspace{-2ex}
\begin{tabular}{l|rr|rr|rr}
 \toprule
       & \multicolumn{1}{c}{RewardRepair} & \multicolumn{1}{c|}{\iFix} & \multicolumn{1}{c}{CURE} & \multicolumn{1}{c|}{\iFix} & \multicolumn{1}{c}{KNOD} & \multicolumn{1}{c}{\iFix} \\ \hline
MEDIAN & 1                                & \textbf{1}                & 1                        & \textbf{1}                & 1                        & \textbf{1}               \\
MEAN    & 4.1                              & \textbf{1.4}              & 3.5                      & \textbf{1.7}              & 2.9                      & \textbf{1.9}             \\  \bottomrule
\end{tabular}
\end{table}

% \begin{table}[]
% \small
% \caption{The number of the correct patch ranks that win, tie, and lose to other APR tools}
% \label{table: win tie lose of different APR}
% \begin{tabular}{lrrr}
%  \toprule
% \multicolumn{1}{l|}{}     & \multicolumn{1}{l}{RewardRepair} & \multicolumn{1}{l}{CURE} & \multicolumn{1}{l}{KNOD} \\ \hline
% \multicolumn{1}{l|}{WIN}  & 10                               & 11                       & 5                        \\
% \multicolumn{1}{l|}{TIE}  & 15                               & 17                       & 34                       \\
% \multicolumn{1}{l|}{LOSE} & 2                                & 3                        & 5                        \\ \hline
% \multicolumn{1}{l|}{TOTAL}                     & 27                               & 31                       & 44                       \\  \bottomrule
% \end{tabular}
% \end{table}

Table~\ref{table: comparison results of APR} shows the mean and median ranking positions of the correct patch produced by our method compared with the default rankings from three APR techniques. Our method consistently improves the default rankings by at least 34\% compared with the three APR techniques. %Table~\ref{table: win tie lose of different APR} shows the number of bugs where our method wins, ties, and loses to the original ranking of the APR techniques.  The results show that our multi-criteria method consistently improves the ranking of correct patches from different APR tools on most bugs. Even though the number of bugs where our method wins is the same as the number it loses to the ranking of KNOD, our method improves the rank of correct patches with an average number of 13.4 while only losing with an average rank of 4.6. 






==> templates/6-UserStudy.tex <==
To evaluate the overall usefulness and usability of \iFix, we conducted a within-subjects user study with 15 participants. This study has been approved by the IRB office at the local university. We investigate the following research questions:

\begin{itemize}[leftmargin=10mm]
    \setlength\itemsep{0.5mm}
    \item[\textbf{RQ3}] How effectively can \iFix help developers select the correct patch from many plausible patches generated by an APR technique?
    \item[\textbf{RQ4}] To what extent does \iFix improve  developers' trust in automatically generated patches?
\end{itemize}

\subsection{Participants and Protocol}
We recruited 15 computer science students who had at least 2--5 years of programming experience. %67\% of them have a Java programming experience of at least one year. Furthermore, 93\% of the participants have been using Visual Studio Code for their daily use for at least one year. 73.3\% of the participants have the experience of using Eclipse, among which 27.3\% have used Eclipse for more than one year.
Similar to the quantitative experiment in Section~\ref{sec:QuantitativeExperiment}, we used CURE~\cite{jiang_cure_2021} as the underlying APR technique in the user study. We selected four bugs from Defects4J that have sufficient plausible patches for developers to explore. Table~\ref{tab:user-study-tasks} shows the details of these bugs. 
For each participant, we selected three bugs and asked the participant to fix them in three settings: (1) manually selecting the correct patch from a list of automatically generated patches (\textit{manual}), (2) selecting the correct patch with the aid of \iFix (\textit{iFix}), and (3) selecting the correct path with the aid of InPaFer, a state-of-the-art interactive patch filtering technique~\cite{liang_interactive_2021}  (\textit{InPaFer}). 


\begin{table} []
% \small
  \caption{Four bugs used for the user study}
  %\vspace{-2ex}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{l|llr}
    \toprule
    \multicolumn{1}{c|}{Bug ID} & \multicolumn{1}{c}{Project Name} & \multicolumn{1}{c}{Root Cause} & \multicolumn{1}{c}{\# of Plausible Patches} 
    \\ 
    \midrule
    Lang 6 & Commons Lang & Wrong argument  & 7 \\
    \hline
    Math 30 & Commons Math & Integer overflow & 33 \\
    \hline
    Chart 9 & JFreeChart & Wrong condition & 22 \\
    \hline
    Math 94 & Commons Math & Integer overflow & 9 \\
    \bottomrule
  \end{tabular}%
  }

  \label{tab:user-study-tasks}
\end{table}


To faithfully represent the real-world usage scenario, participants were allowed to freely edit the code, navigate the codebase, run test cases, and use the default debugger in the IDE in all three settings. 
% We prepared a bug report for each bug to make our participants familiar with the buggy project. The bug reports were designed to withhold the root cause of the bugs, thus encouraging the participants to thoroughly explore possible solutions and make informed decisions.
The task assignment was counterbalanced to mitigate the learning effect. Before using \iFix and InPaFer, participants are provided a tutorial video to learn how to use them. Each task was limited to 30 minutes. At the end of each task, we asked participants to complete a post-task survey, which includes five NASA Task Load Index (TLX) questions~\cite{HART1988139} for assessing the cognitive load (Table \ref{tab:nasa-tlx}), as well as six Likert-scale questions to rate the usefulness of the tool and the cognitive load of using the tool. After all three tasks, they were asked to complete a final survey to directly compare the three settings.
 % and used plausible patches generated by CURE~\cite{jiang_cure_2021}, an advanced APR tool capable of fixing these bugs. To make counter balance, we ensured that the bugs Math 30, Chart 9, and Lang 6 were fixed four times separately across the three sessions, while Math 94 was fixed three times. We evenly distributed bug fixing tasks to our 15 participants based on this constraint.

%We prepared a bug report for each bug to make our participants familiar with the buggy project and class. The bug reports were designed to withhold the root cause of the bugs, thus encouraging the participants to thoroughly explore the possible solutions and make informed decisions when selecting and applying the plausible patches. We set up a time limit of 30 minutes per session. After each session, we asked the participants to complete a post-task survey. They were asked to answer five NASA Task Load Index questions ~\cite{HART1988139} to rate the cognitive load of using the tools, as shown in Table \ref{tab:nasa-tlx}. When all three sessions are finished, we asked them to fill out a final survey to get their feedback on how useful they found the tools we used. 

\begin{table}[]
\small
  \caption{NASA TLX Questions for Cognitive Load Assessment}
% \vspace{-2ex}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{l}
    \toprule
    NASA Task Load Index Questions   \\
    \midrule
    Q1. How mentally demanding was using this tool? \\
    Q2. How hurried or rushed were you during the task?  \\
    Q3. How successful would you rate yourself in accomplishing the task?  \\
    Q4. How hard did you have to work to achieve your level of performance?  \\ 
    Q5. How insecure, discouraged, irritated, stressed, and annoyed were you? \\
    \bottomrule
  \end{tabular}%
  }
  \label{tab:nasa-tlx}
  % \vspace{-2ex}
\end{table}

\subsection{User Study Results}

As shown in Figure \ref{fig:user_completion}, all 15 participants successfully selected the correct patch within the given time when using \iFix. By contrast, 11 and 13 participants selected the correct patch manually and when using InParFer. Table~\ref{tab:user-study-settings} shows the average task completion time. Overall, \iFix consistently reduced the task completion time for all four bugs compared with manual selection and InPaFer. %The average completion time using \iFix was 7.2 minutes, whereas the average completion time using only patches and InPaFer was 11.5 minutes and 11.7 minutes, respectively. 
The mean difference between \iFix and InPaFer (4.5 min) is statistically significant (paired t-test: df = 14, p-value = 0.0068). The mean difference between using \iFix and manual selection (4.3 min) is also statistically significant (paired t-test: df = 14, p-value = 0.0416).


In the post-task survey, 13 of 15 participants agreed or strongly agreed that \iFix was helpful in finding the correct patch, as shown in Figure \ref{fig:user_preference}. By contrast, only 4 participants agreed or strongly agreed that InPaFer was helpful, and none participants agreed or strongly agreed that manual selection was helpful. Furthermore, \iFix significantly enhances developers' confidence in the auto-generated patches. As shown in Figure \ref{fig:user_confidence}, 12 participants agreed or strongly agreed that they felt confident about their patch selection when using \iFix. In contrast, only 6 and 4 participants felt so when using InPaFer and manual selection.   %They felt more confident about the patch selected by \iFix. 
After finishing the manual debugging task, P8 said, ``{\em at the end of this experiment, I am questioning whether the generated patches are correct. In addition, I can not responsibly accept a patch that I did not understand, so I have to rethink of what the patch actually does anyways.}’’ 
% After completing the task using InPaFer, P13 said, ``{\em I don't like it because it is too complex to use. When I try to compare the paths of different patches, I have already understood the code so that I can directly fix the bugs.}’’
Finally, participants also perceived less cognitive effort when using \iFix, as shown in Figure \ref{fig:nasa_tlx}. 
%One of the reasons is that they did not have to distinguish between too much patches. % After finishing the manual debugging task P5 said, ``{\em There are quite a few patches, it took some time to check which one might be the correct one. I would prefer 2 to 3 patches and choose one from them.}’’ P7 said, ``{\em There are too many patches generated and some of them are obviously wrong. However it is quite time consuming for me to check them one by one.}’’ With InPaFer, the participants still need to go over many patches after utilizing the filters. P6 said, ``{\em [When using InPaFer] I totally checked 7 patches and the first 6 are incorrect. I think if I am capable of recognizing the incorrect patches, it will only take me seconds to fix the bug. It actually cost me much more time than I debug it by myself.}


\begin{figure}
    \centering
    \includegraphics[width=0.55\columnwidth]{Figures/user_completion.pdf}
    % \precaptionspace
    %\vspace{-2ex}
    \caption{Task Completion Rate}
    \label{fig:user_completion}
\end{figure}


\begin{table}
\small
  {%
  \caption{Average Task Completion Time in Minutes}
  \label{tab:user-study-settings}
  %\vspace{-2ex}
  \begin{tabular}{c|ccc}
    \toprule
    {Bug ID} & \textit{iFix} & \textit{Manual} & \textit{InPaFer}  \\
    \midrule
    Lang 6 & 6.7 & 17.5 & 15.0 \\
    Math 30 & 8.0 & 8.4 & 12.1 \\
    Chart 9 & 6.9 & 10.8 & 10.8 \\
    Math 94 & 7.1 & 8.7 & 18.1 \\
    \midrule
    Average & 7.2 & 11.5 & 11.7 \\
    \bottomrule
  \end{tabular}%
  }
  
\end{table}

Figure \ref{fig:feature_rating} shows developers' ratings on individual features in {\iFix}. The {\em runtime comparison table} is the most appreciated feature, followed by {\em multi-criteria sampling}, {\em color-highlighting}, and {\em navigation support}. P3 said, ``{\em it [iFix] reduces the number of patches so I can focus more on the given patches and think about them.}'' P2 said, ``{\em [I am] able to see variables in the table. It helps to visualize some corner cases.}''

When selecting patches manually, 7 of our 15 participants utilized the IDE debugger to examine the runtime behavior of a patch. Meanwhile, 5 participants used the IDE debugger when using InPaFer. By contrast, only 1 participant used the IDE debugger when using \iFix. This highlights the effectiveness of the runtime behavior comparison feature in \iFix, which significantly reduces the need for manual debugging in patch assessment.%P13 said, ``{\em I don't like it(InPaFer) because it is too complex to use. When I try to compare the paths of different patches, I have already understood the code so that I can directly fix the bugs.}’’

Participants also identified some drawbacks of \iFix. Like InPaFer, they found \iFix requires some effort to learn. P2 said, ``{\em the learning curve [of iFix] is high.}'' %Sometimes I can fix a bug based on my knowledge and the widgets may distract me.}’’ P6 pointed out a limitation of the design of \iFix, ``{\em It works well for one-line debuggging scenario but I kindly worry about what if there are multiple lines. It may take too much space in my VScode.} 
Participants also suggested some improvement opportunities. P6 said, ``{\em I wish it could explain the trace in a better way, like a workflow chart.}'' P7 expected \iFix to have ``{\em some explanations for the meaning of the proposed patches.}''


% \begin{table*}
%     % \resizebox{0.9\textwidth}{!}{%
%     \newcolumntype{Y}{>{\centering\arraybackslash}X}
%     \begin{tabularx}{0.9\textwidth}{Y||Y|Y|Y||Y|Y|Y||Y|Y|Y||Y|Y|Y}
%     \hline
%     & \multicolumn{3}{c||}{\textbf{Math 94}} & \multicolumn{3}{c||}{\textbf{Math 30}} & \multicolumn{3}{c||}{\textbf{Chart 9}} & \multicolumn{3}{c}{\textbf{Lang 6}} \\
%     \cline{2-13}
%     & \textit{Control} & \textit{iFix} & \textit{InPaFer} & \textit{Control} & \textit{iFix} & \textit{InPaFer} & \textit{Control} & \textit{iFix} & \textit{InPaFer} & \textit{Control} & \textit{iFix} & \textit{InPaFer} \\
%     \hline
%     % Trial 1 &07:05 &05:41 &10:01 &08:03 &07:01 &09:20 &21:54 &04:47 &07:54 &10:49 &06:38 &09:34 \\
%     Trial 1 &\cellcolor{lightpurple!55}07:05 &\cellcolor{lightblue!55}05:41 &\cellcolor{lightcyan!55}10:01 &\cellcolor{lightpurple!55}08:03 &\cellcolor{lightblue!55}07:01 &\cellcolor{lightcyan!55}09:20 &\cellcolor{lightpurple!55}21:54 &\cellcolor{lightblue!55}04:47 &\cellcolor{lightcyan!55}07:54 &\cellcolor{lightpurple!55}10:49 &\cellcolor{lightblue!55}06:38 &\cellcolor{lightcyan!55}09:34 \\
   
%     \hline
%     Trial 2 &07:50 &03:47 &09:20 &08:26 &15:26 &10:49 &08:23 &07:07 &14:54 &08:28 &08:25 &24:48 \\
%     \hline
%     Trial 3 &11:12 &11:51 & - &13:02 &03:24 &16:52 &06:09 &08:22 &10:22 &21:08 &08:09 &18:34 \\
%     \hline
%     Trial 4 & / & / & / &04:12 &05:58 &11:34 & - &07:12 &09:58 &29:35 & -  &07:14 \\
%     \hline
%     Average &08:42 &07:06 &09:41 &08:26 &07:57 &12:09 &12:09 &06:52 &10:47 &17:30 &07:44 &15:03 \\
%     \hline
%     \end{tabularx}
%     % }

%   \caption{Time Consumed on Tasks per Participant (mm:ss) \lin{Why is iFix in the middle? I would put it as the first  or the last} \lin{The way that average is shown as a row makes it hard to see that on average iFix is the best (shortest bug fixing time for users)} }
%   \label{tab:user-study-time}
%   \vspace{-2ex}
% \end{table*}









==> templates/7-Discussion.tex <==
% \todo{talk about limitations. For example, we can only handle single-hunk fixes. We do not consider the side-effects of method calls in def-use analysis.}
%\subsection{Design Implicits}
Our findings suggest that interactive APR techniques should pay more attention to helping developers examine the runtime behavior of patches. As discussed in Section \ref{sec:UserStudy}, 7 of 15 participants used the IDE debugger to investigate the runtime behavior of patches when selecting patches manually. This provides strong evidence for enhancing the debugging experience in the presence of multiple plausible patches. Furthermore, our user study also reveals that only showing basic runtime information without careful design is not sufficient. Specifically, while InPaFer renders the runtime values at the entry and exit of patched methods as well as their execution traces, 5 participants still used IDE debuggers to examine the runtime behavior of patches. By contrast, when using {\iFix}, no participants used IDE debuggers. This implies that the behavior comparison tables with runtime values of variables and expressions related to individual patches are sufficient to help developers understand the root cause of a bug and how it is fixed by different patches. 

%While empirical studies suggested that developers expect fewer candidate patches and more information regarding the bug and the candidate patches~\cite{noller_trust_2022, tao_automatically_2014, winter_lets_2023, winter_how_2022, zhang_program_2022}, our user study revealed from the behavior of developers that they rely on complete runtime information to understand the bug as well as the patches effectively. 


\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/user_preference.pdf}
    % \precaptionspace
    %\vspace{-2ex}
    \caption{The distribution of participants’ preferences}
    \label{fig:user_preference}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/user_confidence.pdf}
    % \precaptionspace
    %\vspace{-2ex}
    \caption{The distribution of participants’ confidence on the selected patches}
    \label{fig:user_confidence}
\end{figure}

%\vspace{-2ex}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{Figures/NASA_TLX.pdf}
    % \precaptionspace

    \caption{Cognitive load measured by NASA TLX~\cite{HART1988139}}
    \label{fig:nasa_tlx}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/feature_rating.pdf}
    % \precaptionspace

    \caption{User ratings on the usefulness of individual features (vertical bar indicating the median)}
    \label{fig:feature_rating}
\end{figure*}

% \subsection{Exploiting Runtime Comparison}
% \label{subsec:exploit}
% The runtime comparison approach has shown wide generalizability. The full stack trace and the per-iteration analysis make it suitable for complex call stacks and control flows. With the design of highlighting different runtime values for the same variable and merging adjacent cells with the same value, it will be much easier for the user to discover the significant statements that could explain the root cause of the bug. 

%The visualization of runtime behavior comparison in \iFix provides a new perspective to distinguish between different patches. Our study revealed that such an approach is helpful for the users to understand the root cause of bugs. The runtime behavior comparison table has the potential to be augmented into more comprehensive forms, e.g., workflow charts and a higher level of explanation of candidate patches in natural language. Moreover, the insight of runtime comparison can be leveraged to enhance the explainability of APR tools, including pattern-, heuristic-, constrain- and deep learning-based APR techniques. It serves as a good starting point for human-in-the-loop automatic program repair. 

% limitations

% \subsection{Threats to Validity}
% \label{subsec:threats}
\vspace{1mm}

\noindent{\bf Threats to Validity}. 
Regarding \textit{internal validity}, the performance of participants in our user study may have been influenced by their programming skills, as well as the difficulty of their task assignments. For example, expert programmers are likely to be more capable of fixing a bug quickly than less experienced ones. To address this bias, we selected participants with diverse levels of Java programming experience and chose four different bugs from Defects4J. We also counterbalanced the task assignment to ensure that each task was experienced by a similar number of participants while mitigating the learning effect in a within-subjects study. %We evenly distributed these tasks into a total of 45 bug fixing sessions, with three sessions assigned to each of the 15 participants. While our scale of debugging sessions (45) and the number of tasks (4) may not be as large as the maximum reported among user studies on APR, our approach is still comparable to most previous studies~\cite{liang_interactive_2021}.

Regarding \textit{external validity}, iFix primarily focuses on Java bugs from the Defects4J dataset. However, some APR techniques are capable of fixing bugs in multiple programming languages~\cite{xia_less_2022}, such as Python and JavaScript. We can address this issue by developing program analysis and code instrumentation methods for different target programming languages at the back end of {\iFix}. This will allow {\iFix} to expand its scope beyond Java and facilitate developers in addressing issues in other programming languages.

Regarding \textit{construct validity}, we chose to focus on bugs with single-hunk patches from the Defects4J dataset for the development of \iFix.  While it is a common practice to select bugs that lie in single-hunk fixing for research purposes~\cite{saha_elixir_2017, le_history_2016, jiang_cure_2021, xia_less_2022}, the interface of iFix could be enhanced to accommodate bugs that require multiple-hunk fixing. One possible solution would be to leverage the split view design to display multiple code locations in a single code editor and leverage color-encoding to show the visual correspondence between different hunks of a patch in different code locations. In this way, developers can view and compare multiple code changes simultaneously.

\vspace{1mm}

\noindent{\bf Limitations and Future Work}. 
\iFix currently focuses on Java bugs with single-hunk patches generated by state-of-the-art APR techniques. In order to improve the generalizability of \iFix, efforts can be made to support bugs with multi-hunk patches and introduce program analysis and instrumentation methods for other programming languages, such as Python and JavaScript. Additionally, the behavior comparison table could be further improved by improving the visual representation of the runtime values, e.g., through a flow chart rather than a comparison table, and incorporating richer information to help developers understand and build trust on automatically generated patches, e.g., a high-level explanation of a patch in natural language. 


==> templates/8-RelatedWork.tex <==
\subsection{Automated Program Repair}
Over the past decade, various APR techniques have been proposed, including pattern-based~\cite{tbar,simfix}, heuristic-based~\cite{arja-heuristic-1,heuristic-2,elixir-heuristic-3}, constrain-based~\cite{ACS-constraint-1,nopol-constraint-2,constraint-3}, and deep learning-based~\cite{chen_sequencer_2019,lutellier_coconut_2020,Li2020dlfix,jiang_cure_2021,hopity,graph2edit,codit,rewardrepair,zhu2021recoder,xia_less_2022} methods. These APR techniques typically follow the generate-and-validate paradigm. That is, they first generate a list of candidate patches by performing different transformations on the buggy code, such as modifying a variable or inserting a function call. They then validate the candidate patches by compiling the patched project and running the test suites. The fixing capability of such APR techniques often suffers from overfitted patches (i.e., incorrect patches that pass the test cases)~\cite{smith_is_2015, le_overfitting_2018}. \iFix is designed as an APR-agnostic approach to improve the usability of APR techniques.  
%Language models have been proved powerful in natural language tasks as well as code generation in the criteria of software engineering. By fine-tuning large models including GPT-3 and BERT, the efficiency of generating code have been boosted a lot. Zimin et al.\cite{chen_sequencer_2019} automated generated patches based on a trained sequence-to-sequence language model in their work SequenceR. CURE\cite{jiang_cure_2021} introduced code-specific generating and searching strategies based on a language model trained with large scale of programming language corpus. Such effort improved the drawback of DL-based APR techniques, which performs lower on the accuracy of generated patches compared with traditional patch generation techniques. CoCoNuT\cite{lutellier_coconut_2020} proposed a novel a Neural Machine Translation model which can represent buggy code and its surrounding context code. Such methodology automates the rule-based patch generation and needs no human effort to create hard code rules, which improved the efficiency in APR tesks. AlphaRepair\cite{xia_less_2022} used a pretrained CodeBERT model to generate correct code at the position of buggy lines. By applying a set of syntax-aware code template, It can generate patches in the manner of real programmers, who often seek changing a certain part in a line of code. AlphaRepair is claimed to perform the state-of-the art on popular program repair benchmarks, including Defects4j and QuixBugs.

\subsection{Human Aspects of APR}
There is a growing interest in studying the usability challenges in APR. Smith et al.~\cite{smith_is_2015} and Le et al.~\cite{ le_overfitting_2018} investigated the overfitting issue in APR, which negatively affects developers' confidence on auto-generated patches. Long et al.~\cite{long_analysis_2016} suggested APR techniques incorporate enriched information into patch generation in order to reduce the search space and generate more precise patches. 

Several studies have been conducted to understand the developer needs and concerns about adopting APR techniques in real-world scenarios~\cite{noller_trust_2022, tao_automatically_2014, winter_lets_2023, winter_how_2022, zhang_program_2022}.  These studies provided substantial insights for research on APR techniques. Recently, several interactive approaches have been proposed to enhance the usability of APR techniques. %One approach involves generating additional test cases to enhance the reliability of patches~\cite{liang_interactive_2021, bohme_2020_human, cashin2019understanding, gao2020interactive}. 
Böhme et al.~\cite{bohme_2020_human} proposed LEARN2FIX, a human-in-the-loop repair technique that elicits developer feedback to guide the patch generation process. LEARN2FIX actively queries developers to build a test oracle before patch generation to overcome the overfitting problem.
Cashin et al.~\cite{cashin2019understanding} proposed to cluster semantically similar patches based on program invariants. Thus, developers ideally only need to examine one patch per cluster.
Gao et al.~\cite{gao2020interactive} proposed an interactive patch suggestion paradigm by translating patch semantics into a set of \textit{what} and \textit{how} questions.
The \textit{what} questions formulated the expected program behaviors, while the \textit{how} questions represented how to modify the program to realize such expected behaviors. 
% \todo{the description below is shallow.}
Liang et al.~\cite{liang_interactive_2021} proposed an interactive patch filtering approach called InPaFer, which helps users filter out incorrect patches based on the bug location, execution traces, and the runtime values at the entry and exit location of buggy methods. Compared to these methods, \iFix not only effectively eliminates the number of candidate patches for users to distinguish, but also fully exploits the runtime information of the bug with different patches by capturing and comparing all related runtime values along the call stack of the buggy or patched code.


\subsection{Differential Testing}
It is expensive to evaluate test results without prior knowledge of expected outputs.
Differential testing address this problem by comparing the output of multiple software systems with similar structures using the same set of inputs \cite{mckeeman1998differential}. Differential testing is well-suited to find semantic or logic bugs that do not exhibit explicit erroneous behaviors.
Daniel et al.~\cite{daniel2007automated} used differential testing to generate Java programs for refactoring engine testing.
Saff et al.~\cite{saff2005automatic} generated unit tests from system tests by recording interactions such as method calls and referenced objects and by introducing wrapper classes to load serialized interactions.
Elbaum et al.~\cite{elbaum2008carving} presented a framework for carving and replaying differential unit tests that accounts for a wide variety of strategies and trade-offs.

More recently, differential testing has been used in finding bugs for deep learning (DL) libraries and compilers. 
Liu et al. proposed $ \nabla $Fuzz \cite{yang2023fuzzing}, which automatically
performs differential testing of each DL library API under different execution scenarios provided by the underlying DL library for each test oracle.
CRADLE \cite{pham2019cradle} was a new approach focusing on finding and localizing bugs in DL software libraries. CRADLE leverages differential testing to detect bugs by running existing DL models on different low-level DL libraries. 
Wang et al. proposed EAGLE \cite{wang2022eagle} that uses equivalent graphs to differentially test DL APIs. 
Liu et al.~\cite{liu2023nnsmith} proposed NNSmith, which finds DL compiler bugs via differential testing. NNSmith synthesizes random models for compilation, runs the compiled models with random inputs, and compares the generated results with those from a reference implementation. In this paper, \iFix organizes the outputs of variables into a run-time behavior comparison table to provide an informative yet intuitive visual representation to help developers find behavior differences among multiple patch candidates.


==> templates/9-Conclusion.tex <==
This paper presents \iFix, an interactive approach that allows developers to quickly explore a large number of patch candidates and examine their behavior difference without manual debugging. \iFix uses a multi-criteria sampling and re-ranking method to select a small set of diverse and representative patches and re-rank them based on their similarity to the buggy code.
Compared with other ranking methods, \iFix improves the overall ranking of the correct patch by at least 34\%. We further demonstrate the generalizability of our method by employing our multi-criteria method by leveraging it on different APR tools.
Moreover, \iFix uses runtime behavior analysis to capture the runtime behavioral differences among buggy and patched code. We have implemented \iFix as a VS Code extension and conducted a within-subjects user study with 15 participants. Our user study shows that compared with manual debugging and a state-of-the-art patch filtering technique, \iFix improves the success rate by 27\% and 14\% while reducing the task completion time by 37\% and 38\%, respectively.
